Exploring Community-Driven Descriptions for Making Livestreams Accessible

People watch livestreams to connect with others and learn about their hobbies. Livestreams feature multiple visual streams including the main video, webcams, on-screen overlays, and chat, all of which are inaccessible to livestream viewers with visual impairments. While prior work explores creating audio descriptions for recorded videos, live videos present new challenges: authoring descriptions in real-time, describing domain-specific content, and prioritizing which complex visual information to describe. We explore inviting livestream community members who are domain experts to provide live descriptions. We first conducted a study with 18 sighted livestream community members authoring descriptions for livestreams using three different description methods: live descriptions using text, live descriptions using speech, and asynchronous descriptions using text. We then conducted a study with 9 livestream community members with visual impairments, who shared their current strategies and challenges for watching livestreams and provided feedback on the community-written descriptions. We conclude with implications for improving the accessibility of livestreams.

==> audience-preferences.tex <==
\begin{table}[]
\begin{tabular}{ccccc}
\toprule
PID      & Main Content & Chat & Cameras & Overlays \\
\midrule
U1       & 1            & 3    & 3       & 2        \\
U2       & 1            & 2    & 3       & 3        \\
U3       & 1            & 1    & 3       & 3        \\
U4       & 1            & 2    & 4       & 3        \\
U5       & 1            & 2    & 3       & 3        \\
U6       & 1            & 2    & 2       & 2        \\
U7       & 1            & 4    & 2       & 2        \\
U8       & 1            & 2    & 2       & 2        \\
U9       & 1            & 4    & 3       & 2        \\
\bottomrule 
Averages & 1            & 2.44 & 2.78    & 2.44    
\caption{Table of ranked order priority for each description focus. Lower number indicates stronger preference. Ties indicate no preference between foci.}
\label{tab:preferences}
\end{tabular}
\end{table}

==> quant.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htp]
\begin{tabular}{@{}llllccrrrr@{}}
\toprule
Session ID & PID & Condition & Category & Video ID & Duration (sec) & \# Desc & \# Words & Desc/Min & Words/Min \\ \midrule
BOTW-C-A & P1 & Audio & Breath of the Wild & V3 & 302 & 51 & 396 & 10.132 & 78.676 \\
Chess-C-A & P2 & Audio & Chess & V6 & 296 & 18 & 118 & 3.649 & 23.919 \\
Chess-B-A & P3 & Audio & Chess & V5 & 371 & 42 & 849 & 6.792 & 137.305 \\
Chess-A-A & P4 & Audio & Chess & V4 & 375 & 12 & 81 & 1.920 & 12.960 \\
Art-A-A & P5 & Audio & Digital Art & V7 & 338 & 19 & 128 & 3.373 & 22.722 \\
Art-C-A & P6 & Audio & Digital Art & V9 & 319 & 22 & 118 & 4.138 & 22.194 \\
Art-B-A & P7 & Audio & Digital Art & V8 & 279 & 16 & 156 & 3.441 & 33.548 \\
League-C-A & P8 & Audio & League of Legends & V12 & 346 & 39 & 299 & 6.763 & 51.850 \\
League-A-A & P9 & Audio & League of Legends & V10 & 341 & 34 & 503 & 5.982 & 88.504 \\
League-B-A & P10 & Audio & League of Legends & V11 & 350 & 34 & 330 & 5.829 & 56.571 \\
Makeup-A-A & P11 & Audio & Makeup & V13 & 355 & 27 & 237 & 4.563 & 40.056 \\
Makeup-B-A & P12 & Audio & Makeup & V14 & 299 & 20 & 213 & 4.013 & 42.742 \\
Smash-A-A & P13 & Audio & Smash Bros. Ultimate & V16 & 358 & 29 & 300 & 4.860 & 50.279 \\
Smash-C-A & P14 & Audio & Smash Bros. Ultimate & V18 & 297 & 42 & 322 & 8.485 & 65.051 \\
Smash-B-A & P15 & Audio & Smash Bros. Ultimate & V17 & 296 & 49 & 575 & 9.932 & 116.554 \\
Valorant-B-A & P16 & Audio & Valorant & V20 & 117 & 25 & 199 & 12.821 & 102.051 \\
Valorant-C-A & P17 & Audio & Valorant & V21 & 329 & 37 & 535 & 6.748 & 97.568 \\
Valorant-A-A & P18 & Audio & Valorant & V19 & 287 & 46 & 263 & 9.617 & 54.983 \\
BOTW-B-TA & P1 & Text-Async & Breath of the Wild & V2 & 213 & 6 & 171 & 1.690 & 48.169 \\
Chess-B-TA & P2 & Text-Async & Chess & V5 & 299 & 10 & 87 & 2.007 & 17.458 \\
Chess-A-TA & P3 & Text-Async & Chess & V4 & 252 & 18 & 223 & 4.286 & 53.095 \\
Chess-C-TA & P4 & Text-Async & Chess & V6 & 299 & 10 & 108 & 2.007 & 21.672 \\
Art-C-TA & P5 & Text-Async & Digital Art & V9 & 285 & 15 & 234 & 3.158 & 49.263 \\
Art-B-TA & P6 & Text-Async & Digital Art & V8 & 273 & 13 & 135 & 2.857 & 29.670 \\
Art-A-TA & P7 & Text-Async & Digital Art & V7 & 142 & 5 & 71 & 2.113 & 30.000 \\
League-A-TA & P8 & Text-Async & League of Legends & V10 & 269 & 24 & 163 & 5.353 & 36.357 \\
League-B-TA & P9 & Text-Async & League of Legends & V11 & 300 & 11 & 248 & 2.200 & 49.600 \\
League-C-TA & P10 & Text-Async & League of Legends & V12 & 330 & 39 & 205 & 7.091 & 37.273 \\
Makeup-B-TA & P11 & Text-Async & Makeup & V14 & 316 & 19 & 186 & 3.608 & 35.316 \\
Makeup-C-TA & P12 & Text-Async & Makeup & V15 & 306 & 15 & 195 & 2.941 & 38.235 \\
Smash-C-TA & P13 & Text-Async & Smash Bros. Ultimate & V18 & 336 & 13 & 187 & 2.321 & 33.393 \\
Smash-B-TA & P14 & Text-Async & Smash Bros. Ultimate & V17 & 281 & 26 & 149 & 5.552 & 31.815 \\
Smash-A-TA & P15 & Text-Async & Smash Bros. Ultimate & V16 & 145 & 25 & 265 & 10.345 & 109.655 \\
Valorant-A-TA & P16 & Text-Async & Valorant & V19 & 293 & 30 & 130 & 6.143 & 26.621 \\
Valorant-B-TA & P17 & Text-Async & Valorant & V20 & 202 & 23 & 339 & 6.832 & 100.693 \\
Valorant-C-TA & P18 & Text-Async & Valorant & V21 & 317 & 29 & 202 & 5.489 & 38.233 \\
BOTW-A-TL & P1 & Text-Live & Breath of the Wild & V1 & 327 & 9 & 156 & 1.651 & 28.624 \\
Chess-A-TL & P2 & Text-Live & Chess & V4 & 277 & 7 & 59 & 1.516 & 12.780 \\
Chess-C-TL & P3 & Text-Live & Chess & V6 & 335 & 25 & 229 & 4.478 & 41.015 \\
Chess-B-TL & P4 & Text-Live & Chess & V5 & 294 & 27 & 180 & 5.510 & 36.735 \\
Art-B-TL & P5 & Text-Live & Digital Art & V8 & 314 & 11 & 133 & 2.102 & 25.414 \\
Art-A-TL & P6 & Text-Live & Digital Art & V7 & 373 & 12 & 86 & 1.930 & 13.834 \\
Art-C-TL & P7 & Text-Live & Digital Art & V9 & 235 & 6 & 95 & 1.532 & 24.255 \\
League-B-TL & P8 & Text-Live & League of Legends & V11 & 294 & 13 & 80 & 2.653 & 16.327 \\
League-C-TL & P9 & Text-Live & League of Legends & V12 & 333 & 16 & 210 & 2.883 & 37.838 \\
League-A-TL & P10 & Text-Live & League of Legends & V10 & 311 & 20 & 123 & 3.859 & 23.730 \\
Makeup-C-TL & P11 & Text-Live & Makeup & V15 & 271 & 13 & 171 & 2.878 & 37.860 \\
Makeup-A-TL & P12 & Text-Live & Makeup & V13 & 288 & 16 & 195 & 3.333 & 40.625 \\
Smash-B-TL & P13 & Text-Live & Smash Bros. Ultimate & V17 & 278 & 8 & 79 & 1.727 & 17.050 \\
Smash-A-TL & P14 & Text-Live & Smash Bros. Ultimate & V16 & 314 & 22 & 82 & 4.204 & 15.669 \\
Smash-C-TL & P15 & Text-Live & Smash Bros. Ultimate & V18 & 293 & 26 & 165 & 5.324 & 33.788 \\
Valorant-C-TL & P16 & Text-Live & Valorant & V21 & 274 & 18 & 65 & 3.942 & 14.234 \\
Valorant-A-TL & P17 & Text-Live & Valorant & V19 & 295 & 19 & 182 & 3.864 & 37.017 \\
Valorant-B-TL & P18 & Text-Live & Valorant & V20 & 315 & 22 & 144 & 4.190 & 27.429 \\ \bottomrule
\end{tabular}
\caption{Information about description quantities written per session, sorted by description condition. One session is a unique 3-tuple between a given video category, video ID, and description condition, respectively. ``Duration (sec)'' refers to the amount of time starting from the first description recorded to the last description recorded. ``\# Desc'' refers to the number of descriptions written in the duration. ``\# Words'' is an aggregate total of the number of words over all descriptions written that session. ``Desc/Min'' is an average number of descriptions per minute over the recorded duration. Similarly, ``Words/Min'' is an average number of aggregate words per minute over the recorded duration.}
\label{tab:quant}
\end{table*}
